Neural Path Hunter: Reducing Hallucination in Dialogue Systems via Path Grounding

Dialogue systems powered by large pre-trained language models (LM) exhibit an innate ability to deliver fluent and natural-looking responses. Despite their impressive generation performance, these models can often generate factually incorrect statements impeding their widespread adoption. In this paper, we focus on the task of improving the faithfulness -- and thus reduce hallucination -- of Neural Dialogue Systems to known facts supplied by a Knowledge Graph (KG). We propose Neural Path Hunter which follows a generate-then-refine strategy whereby a generated response is amended using the k-hop subgraph of a KG. Neural Path Hunter leverages a separate token-level fact critic to identify plausible sources of hallucination followed by a refinement stage consisting of a chain of two neural LM's that retrieves correct entities by crafting a query signal that is propagated over the k-hop subgraph. Our proposed model can easily be applied to any dialogue generated responses without retraining the model. We empirically validate our proposed approach on the OpenDialKG dataset against a suite of metrics and report a relative improvement of faithfulness over dialogue responses by 20.35% based on FeQA (Durmus et al., 2020).

==> background.tex <==
\section{Background}
We consider the case of generating factual and grounded dialogue when presented with an auxilliary structured knowledge repositories. In particular we focus on factoids of knowledge represented as heterogenous or multi-relational graphs $\G = (\V, \E, \R)$, termed Knowledge Graphs (KG). Each KG 
consists of a set of directed edge triples $e=\langle u, r, v \rangle \in \E$, where $u, v \in \V$ are nodes and $r \in \R$ is a relation type. It is well known that KG's while useful are also incomplete ---i.e. there are missing edges between entities, thus predicting missing edges by reasoning over an entity's local neighborhood represents a central task. One such approach to KG completion is through learning lower dimensional embeddings of both entities and relations and then scoring the likelihood of a triple existing under the learned model. Such embedding models can then hope to power downstream applications one of which is dialogue generation and is the focus of this paper. 

\xhdr{Relation Prediction}
The general {\em relation prediction} task on such a  graph is as follows.
Let $\E_{\textrm{train}}\subset \E$ denote a set of observed {\em training} edges and let $\bar{\E} = \{\langle v_i, r, v_j \rangle : v_i, v_j \in \V, r \in R\} \setminus \E$ denote the set of {\em negative} edges that are not present in the true graph $\G$.
Given $\E_{\textrm{train}}$, we aim to learn a scoring function $s$ such that $s(e) > s(e'), \forall e \in \E, e' \in \bar{\E}.$

In other words, the learned scoring function should ideally score any true edge higher than any negative edge. We aim to solve this relation prediction task by learning a function $f_e : \V \mapsto \mathbb{R}^d$ that maps each node $v \in \V$ to an embedding $\mb{z}_v = f_e(v)$. Analogously we may also choose to map each relation $ r \in \R $ to a corresponding embedding, $\mb{z}_r$, via $f_r : \R \mapsto \mathbb{R}^d$. To learn such embedding models it is standard practice to apply contrastive learning methods that make use of a corruption distribution \cite{dyer2014notes,mnih2012fast,ahrabian2020structure,bose2018adversarial}
where the loss over a batch of triples 
$\E_{\textrm{batch}} \subseteq \E_{\textrm{train}}$ is given by:
\begin{equation}\label{eq:genericloss}
    \sum_{e \in \E_{\textrm{edge}}} L_{\textrm{edge}}(s(e), s(e^{-}_1), ..., s(e^{-}_m)),
\end{equation}
where $L_{\textrm{edge}}$ is a per-edge loss function and $e^{-}_1, ..., e^{-}_m \in \bar{\E}$ are ``negative samples'', i.e., randomly sampled edges that do not exist in the graph.
Loss functions of this form generally attempt to maximize the likelihood of true edges compared to the negative samples. 
